The FruitShell French synthesis system at the Blizzard 2023 Challenge

This paper presents a French text-to-speech synthesis system for the Blizzard Challenge 2023. The challenge consists of two tasks: generating high-quality speech from female speakers and generating speech that closely resembles specific individuals. Regarding the competition data, we conducted a screening process to remove missing or erroneous text data. We organized all symbols except for phonemes and eliminated symbols that had no pronunciation or zero duration. Additionally, we added word boundary and start/end symbols to the text, which we have found to improve speech quality based on our previous experience. For the Spoke task, we performed data augmentation according to the competition rules. We used an open-source G2P model to transcribe the French texts into phonemes. As the G2P model uses the International Phonetic Alphabet (IPA), we applied the same transcription process to the provided competition data for standardization. However, due to compiler limitations in recognizing special symbols from the IPA chart, we followed the rules to convert all phonemes into the phonetic scheme used in the competition data. Finally, we resampled all competition audio to a uniform sampling rate of 16 kHz. We employed a VITS-based acoustic model with the hifigan vocoder. For the Spoke task, we trained a multi-speaker model and incorporated speaker information into the duration predictor, vocoder, and flow layers of the model. The evaluation results of our system showed a quality MOS score of 3.6 for the Hub task and 3.4 for the Spoke task, placing our system at an average level among all participating teams.

==> 123.tex <==
The Blizzard Challenge is held once a year, and this year's theme is French synthesis. Participants are required to synthesize French text for two tasks within a limited time frame, using a limited dataset provided by the organizers. 

The two tasks are the Hub task and the Spoke task. The Hub task involves building a voice using the provided French data (NEB) using only publicly available data. The goal is to synthesize a voice that closely resembles the characteristics of the NEB dataset. On the other hand, the Spoke task requires participants to build a voice that is as close as possible to the AD dataset, using the provided French data. 

In recent years, text-to-speech synthesis systems have been a hot topic of research.  The goal of these systems is to take specific input text and generate high-quality, natural-sounding speech audio while trying to make the voice and prosody as close as possible to the desired target. 

Speech synthesis has undergone various evolutions in its technology. The earliest methods involved physical modeling of speech production, simulating the human vocal tract to synthesize speech \cite{1454423,shadle2001prospects}. This was followed by waveform concatenation methods for speech synthesis \cite{1170350,black1998festival}, where audio segments were selected from a database and concatenated to generate speech waveforms. However, this approach required large databases. 

Subsequently, statistical parametric synthesis methods were developed \cite{yoshimura1999simultaneous}. The basic idea was to generate acoustic-related parameters and then recover waveforms from these parameters. 

Over time, researchers have gradually developed methods for speech synthesis using deep neural networks. Initially, partial end-to-end synthesis was performed, where an acoustic model \cite{wang2017tacotron,ren2019fastspeech,li2019neural} generated acoustic features, which were then converted back to waveforms using a vocoder \cite{oord2016wavenet,valin2019lpcnet,kong2020hifi}. However, this approach can accumulate errors between different components, leading to a decrease in synthesis quality. 

To address this issue, researchers have proposed some end-to-end models such as Deep Voice 3 \cite{ping2017deep}, Fastspeech2 \cite{ren2020fastspeech}, GlowTTS \cite{kim2020glow}, and Diffspeech \cite{jeong2021diff}. These models can directly generate the final speech from input text. The aim is to simplify the text analysis module by directly using character/phoneme sequences as input and simplifying acoustic features into magnitude spectra to improve the accuracy of acoustic feature prediction. 

This article will provide a brief overview of an end-to-end approach used for French synthesis in the competition, including the complete process, including data preprocessing. The results of the competition will also be presented at the end. 
